Gaia Gaps and the Physics of Low-Mass Stars. I. The Fully Convective Boundary

The Gaia M-dwarf gap is a significant under-density of stars observed near $M_G = 10.2$ in a color-magnitude diagram for stars within 200 pc of the Sun. It has been proposed that the gap is the manifestation of structural instabilities within stellar interiors due to non-equilibrium $^{3}$He fusion prior to some stars becoming fully convective. To test this hypothesis, we use Dartmouth stellar evolution models, MARCS model atmospheres, and simple stellar population synthesis to create synthetic $M_G$-($G_{\rm BP} - G_{\rm RP})$ color-magnitude diagrams. We confirm that the proposed $^{3}$He instability is responsible for the appearance of the M-dwarf gap. Our synthetic gap shows qualitatively similar features to the observed gap including: its vertical extent in $M_G$, its slope in the color-magnitude diagram, and its relative prominence at bluer colors as compared to redder colors. Furthermore, corresponding over-densities of stars above the gap are reproduced by the models. While qualitatively similar, the synthetic gap is approximately 0.2 magnitudes bluer and, accounting for this color offset, 0.16 magnitudes brighter than the observed gap. Our results reveal that the Gaia M dwarf gap is sensitive to conditions within cores of M dwarf stars, making the gap a powerful tool for testing the physics of M dwarf stars and potentially using M dwarfs to understand the local star formation history.

==> Jao Gap Modeling 1_ Fully Convective Boundary/instability_table.tex <==

\begin{deluxetable*}{c c c c c c c c c l}
    %\tablewidth{2\pagewidth}
    \tablecolumns{10}
    \tablecaption{Properties of the 0.350 $M_\sun$ Model Star in Figure 5 \label{tab:instability_evolution}}
    \tablehead{\colhead{Point} & \colhead{Age} & \colhead{$M_{\rm conv.\ core}$} & \colhead{$M_{\rm conv.\ env.}$} & \colhead{$L_{\star}$} & \colhead{$L_{\rm pp}$} & \colhead{$R_{\star}$} & \colhead{$X( ^3\textrm{He})_{\rm core}$} & \colhead{$T_{\rm core}$} & \colhead{Note} \\
    \colhead{\#} & \colhead{[Gyr]} & \colhead{[$M_{\sun}$]} & \colhead{[$M_{\sun}$]} & \colhead{[$L_{\rm zams}$]} & \colhead{[$L_{\rm zams}$]} & \colhead{[$R_{\rm zams}$]} & \colhead{[$\times 10^{3}$]} & \colhead{[MK]} & \colhead{}}
    \startdata
    1 & 0.284 & 0.014 & 0.212 & 1.000 & 1.014 & 1.000 & 1.18 & 7.89 & Minimum radius ZAMS \\
    2 & 0.309 & 0.016 & 0.215 & 1.000 & 1.021 & 1.000 & 1.30 & 7.90 & 1st $T_{\rm core}$ peak \\
    3 & 2.11  & 0.064 & 0.281 & 1.072 & 1.075 & 1.039 & 3.94 & 7.69 & Pre conv.\ zone merger 1 \\
    4 & 2.17  & 0.009 & 0.224 & 1.034 & 0.876 & 1.017 & 1.23 & 7.77 & Post conv.\ zone merger 1 \\
    5 & 2.31  & 0.021 & 0.223 & 1.017 & 1.018 & 1.009 & 1.82 & 7.85 & 2nd $T_{\rm core}$ peak \\ 
    6 & 3.93  & 0.060 & 0.279 & 1.076 & 1.078 & 1.040 & 4.00 & 7.69 & Pre conv.\ zone merger 2 \\
    7 & 4.04  & 0.000 & 0.350 & 1.078 & 1.079 & 1.041 & 2.09 & 7.68 & Post conv.\ zone merger 2 \\
    8 & 10.4  & 0.000 & 0.350 & 1.091 & 1.092 & 1.045 & 4.16 & 7.67 & Fully convective
    \enddata
\end{deluxetable*}


==> instability_table.tex <==

\begin{deluxetable*}{c c c c c c c c c l}
    %\tablewidth{2\pagewidth}
    \tablecolumns{10}
    \tablecaption{Properties of the 0.350 $M_\sun$ Model Star in Figure 5 \label{tab:instability_evolution}}
    \tablehead{\colhead{Point} & \colhead{Age} & \colhead{$M_{\rm conv.\ core}$} & \colhead{$M_{\rm conv.\ env.}$} & \colhead{$L_{\star}$} & \colhead{$L_{\rm pp}$} & \colhead{$R_{\star}$} & \colhead{$X( ^3\textrm{He})_{\rm core}$} & \colhead{$T_{\rm core}$} & \colhead{Note} \\
    \colhead{\#} & \colhead{[Gyr]} & \colhead{[$M_{\sun}$]} & \colhead{[$M_{\sun}$]} & \colhead{[$L_{\rm zams}$]} & \colhead{[$L_{\rm zams}$]} & \colhead{[$R_{\rm zams}$]} & \colhead{[$\times 10^{3}$]} & \colhead{[MK]} & \colhead{}}
    \startdata
    1 & 0.284 & 0.014 & 0.212 & 1.000 & 1.014 & 1.000 & 1.18 & 7.89 & Minimum radius ZAMS \\
    2 & 0.309 & 0.016 & 0.215 & 1.000 & 1.021 & 1.000 & 1.30 & 7.90 & 1st $T_{\rm core}$ peak \\
    3 & 2.11  & 0.064 & 0.281 & 1.072 & 1.075 & 1.039 & 3.94 & 7.69 & Pre conv.\ zone merger 1 \\
    4 & 2.17  & 0.009 & 0.224 & 1.034 & 0.876 & 1.017 & 1.23 & 7.77 & Post conv.\ zone merger 1 \\
    5 & 2.31  & 0.021 & 0.223 & 1.017 & 1.018 & 1.009 & 1.82 & 7.85 & 2nd $T_{\rm core}$ peak \\ 
    6 & 3.93  & 0.060 & 0.279 & 1.076 & 1.078 & 1.040 & 4.00 & 7.69 & Pre conv.\ zone merger 2 \\
    7 & 4.04  & 0.000 & 0.350 & 1.078 & 1.079 & 1.041 & 2.09 & 7.68 & Post conv.\ zone merger 2 \\
    8 & 10.4  & 0.000 & 0.350 & 1.091 & 1.092 & 1.045 & 4.16 & 7.67 & Fully convective
    \enddata
\end{deluxetable*}

